Distributed Real-Time Emulation of Formally-Defined Patterns for Safe Medical Device Control

Safety of medical devices and of their interoperation is an unresolved issue causing severe and sometimes deadly accidents for patients with shocking frequency. Formal methods, particularly in support of highly reusable and provably safe patterns which can be instantiated to many device instances can help in this regard. However, this still leaves open the issue of how to pass from their formal specifications in logical time to executable emulations that can interoperate in physical time with other devices and with simulations of patient and/or doctor behaviors. This work presents a specification-based methodology in which virtual emulation environments can be easily developed from formal specifications in Real-Time Maude, and can support interactions with other real devices and with simulation models. This general methodology is explained in detail and is illustrated with two concrete scenarios which are both instances of a common safe formal pattern: one scenario involves the interaction of a provably safe pacemaker with a simulated heart; the other involves the interaction of a safe controller for patient-induced analgesia with a real syringe pump.

==> eptcsdata.tex <==
\providecommand{\firstpage}{158}
\providecommand{\publicationstatus}{P. C. \"Olveczky (Ed.): First International Workshop on\\
Rewriting Techniques for Real-Time Systems (RTRTS'10)\\
EPTCS 36, 2010, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.36.9}{10.4204/EPTCS.36.9}}

